Cap2Aug: Caption guided Image to Image data Augmentation

Visual recognition in a low-data regime is challenging and often prone to overfitting. To mitigate this issue, several data augmentation strategies have been proposed. However, standard transformations, e.g., rotation, cropping, and flipping provide limited semantic variations. To this end, we propose Cap2Aug, an image-to-image diffusion model-based data augmentation strategy using image captions as text prompts. We generate captions from the limited training images and using these captions edit the training images using an image-to-image stable diffusion model to generate semantically meaningful augmentations. This strategy generates augmented versions of images similar to the training images yet provides semantic diversity across the samples. We show that the variations within the class can be captured by the captions and then translated to generate diverse samples using the image-to-image diffusion model guided by the captions. However, naive learning on synthetic images is not adequate due to the domain gap between real and synthetic images. Thus, we employ a maximum mean discrepancy (MMD) loss to align the synthetic images to the real images for minimizing the domain gap. We evaluate our method on few-shot and long-tail classification tasks and obtain performance improvements over state-of-the-art, especially in the low-data regimes.

==> Sec/background.tex <==
\section{Background}
\label{sec:background}

\textbf{Diffusion models.} Diffusion models~\cite{ho2020denoising, nichol2021glide, ramesh2022hierarchical, rombach2022high} are text-to-image generative models that generate realistic images from free-form texts. Compared to other generative models, e.g, GANs~\cite{goodfellow2020generative}, flow-based models~\cite{kobyzev2020normalizing}, diffusion models produce more diverse and realistic images.  In this work, we consider the stable diffusion~\cite{rombach2022high} a text-guided image-to-image diffusion model. The goal is to update the input image according to the given text prompt. In a diffusion model, Gaussian noise is gradually added to an input image and a denoising autoencoder is trained to reverse the noising process. To learn the data distribution, the denoising autoencoder minimizes the variational lower bound of the data distribution. Due to the Gaussian noise assumption, the loss can be expressed in a closed form and efficient sampling strategies can be utilized. 
Instead of applying the diffusion process on image space, Rombach et al.~\cite{rombach2022high} propose to project the high-dimensional input to low-dimensional latent space for fast and efficient computation. For text-guided image generation, a text-specific encoder is used that projects texts to an intermediate representation and is jointly trained with the denoising autoencoder.


% In this work, we consider the stable diffusion~\cite{rombach2022high}.
% We start with an input image $x$ and gradually add Gaussian noise to generate a noisy image $x_t$. Then a denoising autoencoder is trained to recover the original data by reversing the noising process. Since the goal is to learn the data distribution $p(x)$, the denoising autoencoder is trained to minimize the variational lower bound of $p(x)$. Due to the Gaussian noise assumption, these models can be represented as an equally weighted sequence of denoising autoencoder ($\epsilon_{\theta} (x_t, t)$) corresponding to each denoising step $t = 1, .., T$. Therefore, the corresponding objective function can be expressed as, 
% \begin{equation}
%     L_{DM} = \mathbb{E}_{x, \epsilon \sim \mathcal{N}(0,1),t} [ || \epsilon - \epsilon_{\theta}(x_t, t)||_{2}^{2} ] 
% \end{equation}

% Instead of applying the diffusion process on the high-dimensional input, Rombach et al.~\cite{rombach2022high} propose to project inputs to a lower latent dimension representation and apply diffusion on this. Let's denote the latent space is $z_t = G(x_t)$, where $G(.)$ is the UNet-style encoder \cite{ronneberger2015u}. Then the latent diffusion loss is given as
% %
% \begin{equation}
%     L_{LDM} = \mathbb{E}_{G(x), \epsilon \sim \mathcal{N}(0,1),t} [ || \epsilon - \epsilon_{\theta}(z_t, t)||_{2}^{2} ] 
% \end{equation}
% %
% For text-conditioned image generation, a domain-specific encoder is used ($\tau_{\theta}$) which projects class names ($y$) to an intermediate representation that is mapped to the intermediate layers of the UNet \cite{ronneberger2015u} via a cross-attention layer. Finally, the text-conditional diffusion model is trained jointly using the loss~\cite{rombach2022high} as
% %
% \begin{equation}
%     L_{LDM} = \mathbb{E}_{G(x),y,\epsilon \sim \mathcal{N}(0,1),t} [ || \epsilon - \epsilon_{\theta}(z_t, t, \tau_{\theta}(y))||_{2}^{2} ] 
% \end{equation}
%

\begin{figure}[t]
  \centering
   \includegraphics[scale=0.45]{figure/method_diagram.pdf}
   \caption{Overview of Cap2Aug. We generate captions from the real images using the BLIP caption model~\cite{li2022blip}. The generated captions and real images are fed to the image-to-image diffusion model~\cite{rombach2022high} to generate abundant synthetic images. We then align the synthetic images with the real images to reduce the domain gap. Finally, the combined set of limited real images and aligned synthetic images are used to learn a classifier for the novel class.}
   \label{fig:teaser}
\end{figure}

\textbf{Stable diffusion.} Stable diffusion is a diffusion model conditioned on text embedding of CLIP ViT-L/14~\cite{radford2021learning} text encoder and trained on LAION-400M dataset~\cite{rombach2022high} of image-text pairs. The stable diffusion model can generate  realistic images from text descriptions.
In this work, the stable diffusion model is conditioned on the text prompts that are based on the diffusion-denoising mechanism proposed by SDEdit~\cite{meng2021sdedit}. The method generates/updates images by iterative denoising through a stochastic differential equation conditioned on the encoded version of the text prompt. 
Examples of the input image and caption pairs and corresponding generated images are shown in Fig.~\ref{fig:teaser_fig}.


% Therefore, we pass the novel class names ($y^{novel}$) as text prompts to the stable diffusion to generate semantically meaningful synthetic images ($x^{syn}$). Some examples of the realistic generated synthetic images are shown in Fig.~\ref{fig:cub_images}.

\textbf{Caption models.}
Captions capture the semantic information of an image in a succinct text. Current large-scale vision and language  methods, e.g., CLIP~\cite{radford2021learning}, BLIP~\cite{li2022blip} achieve impressive performance in image captioning. We use the bootstrapping language-image pretraining (BLIP)~\cite{li2022blip} in this work. This framework utilizes the noisy web data by bootstrapping the captions, where a captioner generates synthetic captions and a filter removes the noisy ones.

\textbf{Domain Adaptation using Maximum Mean Discrepancy (MMD).}
Maximum Mean Discrepancy (MMD) loss is frequently used for domain adaptation. Here we briefly summarize the concept.
Let's assume, given a source ($\mathcal{D}_s$) and target domain ($\mathcal{D}_t$), samples are drawn from these domains with the distribution $P$ and $Q$, respectively over a set $\mathcal{X}$. The features of the samples from these domains are denoted as $\{z_{i}^s\}$ and $\{z_{i}^t\}$, respectively. A multi-kernel MMD ($D_{k}(P,Q)$) between probability distributions $P$ and $Q$ is defined as~\cite{long2015learning}: $D_k(P,Q) = || \mathbb{E}_{p} [\psi(z^s)] - \mathbb{E}_{q} [\psi(z^t)] ||_{\mathcal{H}_{k}}^{2}$
% \begin{equation}
%     D_k(P,Q) = || \mathbb{E}_{p} [\psi(z^s)] - \mathbb{E}_{q} [\psi(z^t)] ||_{\mathcal{H}_{k}}^{2}
% \end{equation}
 where $k$ is the kernel function in the functional space, i.e., 
 $ k = \sum_{p=1}^{P} \alpha_{p} k_p$,
 % \begin{equation}
 %      k = \sum_{p=1}^{P} \alpha_{p} k_p
 % \end{equation}
where $k_p$ is a single kernel. The feature map $\psi : \mathcal{X} \rightarrow \mathcal{H}_{k}$ maps into a reproducing kernel Hilbert space. 
$k = \{ \mathcal{N}(0, 0.5), \mathcal{N}(0, 1), \mathcal{N}(0, 2) \}$. If the kernel is \mbox{$k(x,y) = <\psi(x),\psi(y)>_{\mathcal{H}_k}$}, then using kernel trick, MMD can be estimated as without directly learning $\psi(\cdot)$ as:
\begin{multline}
     \bar{D}_k(P,Q) = \frac{1}{n_s^2} \sum_{i=1}^{n_s} \sum_{j=1}^{n_s} k(z_i^s, z_j^s) 
                    + \frac{1}{n_t^2} \sum_{i=1}^{n_t} \sum_{j=1}^{n_t} k(z_i^t, z_j^t) \\
                    - \frac{2}{n_s n_t} \sum_{i=1}^{n_s} \sum_{j=1}^{n_t} k(z_i^s, z_j^t)   
\end{multline}



% \textbf{Mixup Approaches.}
% These are simple yet effective regularization techniques for training deep networks. Several variants of mixup have been proposed in the literature, viz., input mixup~\cite{zhang2017mixup}, cutmix~\cite{yun2019cutmix}, manifold-mixup~\cite{verma2019manifold}, etc. Manifold mixup uses feature level mixup, which provides smoother decision boundary and flattened class representations. Mangla et al.~\cite{mangla2020charting} use manifold mixup for few-shot learning from a regularization perspective. In contrast to the above methods, we are using manifold mixup to tackle the data scarcity problem in few-shot learning by generating more samples.




% \section{Problem Formulation} 

% Following the standard practice, we formulate the few-shot classification problem as follows. We assume access to a large-scale labeled base dataset and the goal is to classify novel classes using a limited set of training images from the novel set. The task is to learn feature representations using the base dataset with abundant samples and then adapt to classify novel classes using only a few samples.

% We denote the base dataset as \mbox{$\mathcal{D}^{\texttt{base}} = \{ x_{t}^{\texttt{base}}, y_{t}^{\texttt{base}} \}_{t=1}^{N^{\texttt{base}}}$}, where $x_{t}^{\texttt{base}}$ is an image from base classes and the corresponding label is $y_{t}^{\texttt{base}} \in C^{\texttt{base}}$. Similarly, we denote the novel dataset as \mbox{$\mathcal{D}^{\texttt{novel}} = \{ x_{t}^{\texttt{novel}}, y_{t}^{\texttt{novel}} \}_{t=1}^{N^{\texttt{novel}}}$}, where $x_{t}^{\texttt{novel}}$ is an image of novel classes and the corresponding label is $y_{t}^{\texttt{novel}} \in C^{\texttt{novel}}$. The base classes and novel classes are disjoint, i.e., $C^{\texttt{base}} \cap C^{\texttt{novel}} = \emptyset$, and usually $|C^{\texttt{base}}| \geq |C^{\texttt{novel}}|$.

% The training and testing are performed in episodes on the novel class images. Each episode $i$ addresses an $N$-way $K$-shot problem where the few-shot classifier is trained on a support set, i.e., \mbox{$\mathcal{D}_{i}^{\texttt{support}} = \{ x_{i,t}^{\texttt{support}}, y_{i,t}^{\texttt{support}} \}_{t=1}^{NK}$} to classify $N$ novel classes containing $K$ images per class. Then, the few-shot classifier is evaluated on a query set \mbox{$\mathcal{D}_{i}^{\texttt{query}} = \{ x_{i,t}^{\texttt{query}}, y_{i,t}^{\texttt{query}} \}_{t=1}^{NK}$} to classify the same $N$ classes. $K$ is usually set to 1 and 5 for 1-shot and 5-shot setups, respectively and $N$ is usually set to 5. 



==> Sec/supple.tex <==
%%%%%%%%% BODY TEXT
\section*{List of contents}

In the supplementary material, we provide more details of our approach, evaluations, and visualizations. The main sections are as listed below.

\begin{enumerate}
    \item Training details.
    \item Ablation studies.
    \item Visualization of synthetic images.
    \item Failure analysis.
    \item tSNE visualization of the embedding space.
\end{enumerate}

\section{Training details}

In our experiments, we have used an NVIDIA A5000 workstation with 24GB GPU memory. Training details and hyperparameters for our experiments are provided in Table.~\ref{table:hparams}.


%%%%%%%%%% hparmas %%%%%%%%%%%%%%%%%%%%%
\begin{table}[!h]
\begin{center}
\caption{Hyperparamters }
\label{table:hparams}
\scalebox{0.8}{
\begin{tabular}{l|l}
\hline\noalign{\smallskip}
Hyperparameters & Values\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\noalign{\smallskip}
Batchsize & 128\\
Learning rate &  0.001 \\
Optimizer &  AdamW \\
Stable diffusion model checkpoint & ``stable diffusion v1-5 model''\\
Residual ratio  & 1 \\
Sharpness ratio & 5.5 \\
strength (diffusion model) & 0.5 \\
guidance scale (diffusion model) & 7.5\\
BLIP-model (caption) & ``blip-image-captioning-large'' \\
\hline 
\end{tabular}}
\end{center}
\end{table}
%%%%%%%%%%%% 




\section{Ablation studies}

\subsection{ Ablation on our proposed contributions}

In this section, we provide the ablation studies of our proposed methods for OxfordPets, OxfordFlowers, FGVC, StanfordCars, Food101, and DTD datasets in Table.~\ref{tab:ablation_mmd_pets_flowers_fgvc} and Table.~\ref{tab:ablation_mmd_cars_food_dtd} respectively. The results verify that including synthetic images along with MMD loss provides best performance and consistently outperform the state-of-the-art.


\subsection{Ablation on coefficient of MMD loss ($\alpha$)}

In this section, we present the results of ablation studies for the important hyperparameters in our approach. 
Specifically, we observe that when the coefficient of MMD loss ($\alpha$) varies, the classification performance changes.
We show the ablation of $\alpha$ for OxfordPets, OxfordFlowers, FGVC, StanfordCars, Food101, and DTD datasets in Table.~\ref{tab:ablation_alpha_pets_flower_fgvc} and Table.~\ref{tab:ablation_alpha_cars_food_dtd} respectively. 

\section{Visualization of synthetic images}

In this section, we provide some of the visualization of the synthetic images generated by Cap2Aug as shown in Fig.~\ref{fig:supple_examples} for OxfordFlower dataset. The generated images look semantically useful edited versions of the real images and therefore will be considered as useful augmentations. The caption guidance helps to generate diverse synthetic images.


\section{Failure Analysis}

Here we show some of the failure cases incurred by our method as shown in Fig.~\ref{fig:supple_failures}. The images generated for ``falafel'' are not similar to actual ``falafel'' class images, rather it generates images of other food category. The model could be confused while generating the images due to either not having enough information of the ``falafel'' class or it confuses with other food items. 
Similarly, for the cases of ``matted texture'' or ``stop sign'' the failure cases are also shown. 
% The potential reason in the case of ``matted texture'' could be the difficulty to explain dynamical texture details using captions. 

\section{tSNE visualization of the embedding space}

We have also performed the t-SNE analysis of the features for EuroSAT and OxfordPets dataset in Fig.~\ref{fig:eurosat_tsne} and Fig.~\ref{fig:pets_tsne} respectively. The tSNE plots reveal that the few-shot learner is learning discriminative representations over iterations. 

\begin{table*}[]
  \centering
  \caption{Ablation on MMD coefficient $\alpha$}
  \scalebox{0.97}{
  \begin{tabular}{@{}lccccccccccccc@{}}
    \toprule
    {} & \multicolumn{4}{c}{\textbf{OxfordPets}} & \multicolumn{4}{c}{\textbf{OxfordFlowers}} & \multicolumn{4}{c}{\textbf{FGVC}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    {\textbf{$\alpha$}} & {2} & {4} & {8} & {16} & {2} & {4} & {8} & {16} & {2} & {4} & {8} & {16}  \\
    \toprule 
    {0 } & {86.94} & {87.35} & {88.19} & {88.98} & {82.86} & {86.19} & {88.46} & {88.22} & {23.10} & {24.18} & {28.80} & {30.87} \\
    {0.01} & {\textbf{87.22}} & {87.89} & {88.19} & {89.58} & {\textbf{83.06}} & {85.83} & {88.55} & {88.18} & {23.07} & {24.06} & {29.25} & {30.73} \\
    {0.1} & {87.16} & {87.84} & {88.17} & {\textbf{89.58}} & {82.86} & {86.43} & {88.51} & {88.22}  & {23.31} & {\textbf{24.87}} & {29.67} & {33.81} \\
    {1} & {87.08} & {\textbf{87.95}} & {\textbf{88.22}} & {89.56} & {82.01} & {\textbf{86.64}} & {\textbf{88.79}} & {\textbf{89.36}} & {\textbf{23.76}} & {24.63} & {\textbf{29.82}} & {\textbf{34.38}} \\
\bottomrule
  \end{tabular}}
  \label{tab:ablation_alpha_pets_flower_fgvc}
\end{table*}


\begin{table*}[]
  \centering
  \caption{Ablation on MMD coefficient $\alpha$}
  \scalebox{0.97}{
  \begin{tabular}{@{}lccccccccccccc@{}}
    \toprule
    {} & \multicolumn{4}{c}{\textbf{StanfordCars}} & \multicolumn{4}{c}{\textbf{Food101}} & \multicolumn{4}{c}{\textbf{DTD}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    {\textbf{$\alpha$}} & {2} & {4} & {8} & {16} & {2} & {4} & {8} & {16} & {2} & {4} & {8} & {16}  \\
    \toprule 
    {0 } & {61.02} & {64.15} & {68.61} & {73.46} & {77.45} & {77.7} & {78.19} & {78.94} & {54.31} & {59.16} & {63.41} & {64.95} \\
    {0.01} & {60.60} & {64.58} & {\textbf{69.01}} & {73.52} & {77.46} & {77.89} & {\textbf{78.45}} & {78.82} & {54.43} & {59.22} & {\textbf{63.47}} & {65.30} \\
    {0.1} & {60.52} & {64.37} & {68.90} & {73.53} & {77.61} & {77.71} & {78.26} & {\textbf{78.97}}  & {\textbf{54.49}} & {\textbf{59.27}} & {63.29} & {\textbf{66.13}} \\
    {1} & {\textbf{61.24}} & {\textbf{64.70}} & {68.63} & {\textbf{74.79}} & {\textbf{77.61}} & {\textbf{77.93}} & {78.30} & {78.75} & {54.25} & {58.62} & {62.88} & {66.07} \\
\bottomrule
  \end{tabular}}
  \label{tab:ablation_alpha_cars_food_dtd}
\end{table*}



\begin{table*}[]
  \centering
  \caption{Ablation Study on contributions}
  \scalebox{0.9}{
  \begin{tabular}{@{}lccccccccccccc@{}}
    \toprule
    {} & \multicolumn{4}{c}{\textbf{OxfordPets}} & \multicolumn{4}{c}{\textbf{OxfordFlowers}} & \multicolumn{4}{c}{\textbf{FGVC}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    {\textbf{Shots}} & {2} & {4} & {8} & {16} & {2} & {4} & {8} & {16} & {2} & {4} & {8} & {16}  \\
    \toprule 
    {Tip-F~\cite{zhang2022tip}} & {87.03} & {87.54} & {88.09} & {89.70} & {82.30} & {85.83} & {90.51} & \textbf{{94.80}} & {23.19} & {24.80} & {29.21} & {34.55} \\
    {Tip-F + Syn} 
    & {87.16} & {87.60} & {88.19} & {89.70} 
    & {82.86} & {86.19} & {90.89} & {94.32}
    & {23.23} & {24.80} & {29.50} & \textbf{{34.58}} \\
    {Tip-F + Syn + MMD} & \textbf{{87.33}} & \textbf{{87.92}} & \textbf{{88.20} }& \textbf{{89.73}} & \textbf{{83.06}} & \textbf{{86.64}} & \textbf{{91.44}} & {94.51}  & \textbf{{23.76}} & \textbf{{24.87}} & \textbf{{29.82}} & {34.38} \\  
\bottomrule
  \end{tabular}}
  \label{tab:ablation_mmd_pets_flowers_fgvc}
\end{table*}


\begin{table*}[]
  \centering
  \caption{Ablation Study on contributions}
  \scalebox{0.9}{
  \begin{tabular}{@{}lccccccccccccc@{}}
    \toprule
    {} & \multicolumn{4}{c}{\textbf{StanfordCars}} & \multicolumn{4}{c}{\textbf{Food101}} & \multicolumn{4}{c}{\textbf{DTD}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
    {\textbf{Shots}} & {2} & {4} & {8} & {16} & {2} & {4} & {8} & {16} & {2} & {4} & {8} & {16}  \\
    \toprule 
    {Tip-F~\cite{zhang2022tip} } & {61.10} & {64.50} & {68.25} & {74.15} & {77.60} & {77.80} & {78.10} & {79.00}  & {53.72} & {57.39} & {62.70} & {65.50} \\
    {Tip-F + Syn} 
    & {61.20} & {64.60} & {68.61} & {74.46}
    & {77.45} & {77.70} & {78.19} & {78.94}
    & {54.31} & {59.16} & {63.41} & {65.95} \\
    {Tip-F + Syn + MMD} & {\textbf{61.25}} & {\textbf{64.70}} & {\textbf{69.15}} & {\textbf{74.80}} & {\textbf{77.66}} & {\textbf{77.89}} & {\textbf{78.47}} & {\textbf{79.05}} & {\textbf{54.50}} & {\textbf{59.28}} & {\textbf{63.47}} & {\textbf{66.13}} \\ 
\bottomrule
  \end{tabular}}
  \label{tab:ablation_mmd_cars_food_dtd}
\end{table*}


\begin{figure*}[]
  \centering
   \includegraphics[scale=0.55]{figure/pets_tsne.pdf}
   \caption{tSNE plot for the image representations across training iterations (left to right) for OxfordPets dataset in 16-shot setting. As training progresses, the representations become more clustered showing the discriminative power of the few-shot classifier.}
   \label{fig:pets_tsne}
\end{figure*}


\begin{figure*}[t]
  \centering
   \includegraphics[scale=0.7]{figure/eurosat_tsne_2.pdf}
   \caption{tSNE plot for the image representations across training iterations (left to right) for EuroSAT dataset in 16-shot setting. As training progresses, the representations become more clustered showing the discriminative power of the few-shot classifier.}
   \label{fig:eurosat_tsne}
\end{figure*}


\begin{figure*}[t]
  \centering
   \includegraphics[scale=0.7]{figure/supple_examples.pdf}
   \caption{Examples of synthetic images generated from real images}
   \label{fig:supple_examples}
\end{figure*}


\begin{figure*}[t]
  \centering
   \includegraphics[scale=0.6]{figure/supple_failure.pdf}
   \caption{Failure cases: The corresponding class names are provided. The synthetic images generated for classes ``Falafel'' from Food101 dataset, ``matted texture'' from DTD dataset and ``Stop Sign'' from Caltech-101 dataset are shown here as some of the failure cases.}
   \label{fig:supple_failures}
\end{figure*}



